Near-Optimum Online Ad Allocation for Targeted Advertising

Motivated by Internet targeted advertising, we address several ad allocation problems. Prior work has established these problems admit no randomized online algorithm better than $(1-\frac{1}{e})$-competitive (\cite{karp1990optimal,mehta2007adwords}), yet simple heuristics have been observed to perform much better in practice. We explain this phenomenon by studying a generalization of the bounded-degree inputs considered by Buchbinder et al.~\cite{buchbinder2007online}, graphs which we call $(k,d)-bounded$. In such graphs the maximal degree on the online side is at most $d$ and the minimal degree on the offline side is at least $k$. We prove that for such graphs, these problems' natural greedy algorithms attain competitive ratio $1-\frac{d-1}{k+d-1}$, tending to \emph{one} as $d/k$ tends to zero. We prove this bound is tight for these algorithms. Next, we develop deterministic primal-dual algorithms for the above problems achieving competitive ratio $1-(1-\frac{1}{d})^k>1-\frac{1}{e^{k/d}}$, or \emph{exponentially} better loss as a function of $k/d$, and strictly better than $1-\frac{1}{e}$ whenever $k\geq d$. We complement our lower bounds with matching upper bounds for the vertex-weighted problem. Finally, we use our deterministic algorithms to prove by dual-fitting that simple randomized algorithms achieve the same bounds in expectation. Our algorithms and analysis differ from previous ad allocation algorithms, which largely scale bids based on the spent fraction of their bidder's budget, whereas we scale bids according to the number of times the bidder could have spent as much as her current bid. Our algorithms differ from previous online primal-dual algorithms, as they do not maintain dual feasibility, but only primal-to-dual ratio, and only attain dual feasibility upon termination. We believe our techniques could find applications to other well-behaved online packing problems.

==> equal-bids-lower-bound.tex <==
\section{Proof of Theorem \ref*{thm:equal-bids} - Equal Bids Case}
\label{sec:equal-bids}
\textbf{Theorem \ref{thm:equal-bids}}
	Algorithm \ref{alg:primal-dual-ad-allocation} with a correct choice of $C$ gains revenue $\left(1-(1-\frac{1}{d})^k\right)\cdot \sum_i B_i$, and is therefore $\left(1-(1-\frac{1}{d})^k\right)$-competitive for the equal-bid ad allocation problem on $(k,d)$-graphs.

\begin{proof}	
The algorithm's primal feasibility is trivial. We choose $C$ ensuring dual feasibility and bound the dual to primal change for each $j$ by $1+C$. As our dual solution will have value $\sum_i B_i$, this implies a revenue of $\left(1/(1+C)\right)\cdot \sum_i B_i$. Optimizing over $C$ yields the claimed bound.

\textbf{Dual change:} As all increases of the dual cost can be credited to previous increases in variables $\{z_i^c\}$, we bound increases in $\sum_i z_i^c\cdot B_i$. Let $j$ be some ad slot and $i$ be its offline match according to Algorithm \ref{alg:primal-dual-ad-allocation}. The change to the primal revenue is $\Delta P=b_i$. But by our choice of $j$'s match and the bound on the size of $j$'s neighborhood ($d(j)\leq d$), the change to the dual cost satisfies 
\[
\begin{array}{ll}
\Delta D &\leq (b_i/B_i - z_i^c)\cdot B_i + \sum_{i'\in N(j)\setminus\{i\}}\left(\frac{1}{d-1}\right) \cdot (z_{i'}^c+C\cdot b_{i'}/B_{i'})\cdot B_{i'} \\

& \leq b_i - z_i^c\cdot B_i + (d-1)\cdot \left(\frac{1}{d-1}\right)\cdot(z_{i} ^c \cdot B_{i}+C\cdot b_{i}) \\
& \leq (1+C)\cdot b_{i}
\end{array}
\]

\textbf{Dual feasibility and dual value:} We can verify by induction that if $d^c(i)$ denotes the number of edges of $i$'s current copy (that is, $i$'s edges since $z_i^c$ was last nullified), then 
\begin{equation*}
z_i^c=C\cdot \frac{b_i}{B_i} \cdot\left(\left(\frac{d}{d-1}\right)^{d^c(i)}-1\right).
\end{equation*}
If $C=1/\big(\big(\frac{d}{d-1}\big)^k-1\big)$ then after at most $k$ edges are added to $i$'s current copy it is matched or $z_i^c=b_i/B_i$, either of which cause $z_i$ to increase by $b_i/B_i$. As observed above, $d(i)\geq k\cdot B_i/b_i$, and so after all the neighbors of $i$ arrive, $z_i$ is at least one. This implies dual feasibility and dual value $D\geq\sum_iB_i$.
This $C$ yields the claimed bound, namely $P\geq \big(\frac{1}{1+C}\big)\cdot D \geq \big(1-\big(1-\frac{1}{d}\big)^k\big)\cdot \sum_i B_i$. 
\end{proof}


==> randomized-algorithms-description.tex <==
\section{Simple Randomized Algorithms Discussed In The Paper}
\begin{algorithm}
	\caption{\textsc{random}}
	\begin{algorithmic}[1]
		\medskip
		\FORALL{$j\in R$}
		\IF{$j$ has a feasible neighbor $i$}
		\STATE match $j$ to a feasible neighbor $i$ chosen uniformly at random
		\ENDIF
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

\begin{algorithm}
	\caption{\textsc{ranking}}
	\begin{algorithmic}[1]
		\medskip
		\STATE \textbf{Init:} Choose a random permutation of $L$, $\sigma\in S_{|L|}$.
		\FORALL{$j\in R$}
		\IF{$j$ has an unmatched neighbor $i$}
		\STATE match $j$ to an unmatched neighbor $i$ minimizing $\sigma(i)$
		\ENDIF
		\ENDFOR
	\end{algorithmic}
\end{algorithm}

